"Can't Take the Pressure?": Examining the Challenges of Blood Pressure Estimation via Pulse Wave Analysis

The use of observed wearable sensor data (e.g., photoplethysmograms [PPG]) to infer health measures (e.g., glucose level or blood pressure) is a very active area of research. Such technology can have a significant impact on health screening, chronic disease management and remote monitoring. A common approach is to collect sensor data and corresponding labels from a clinical grade device (e.g., blood pressure cuff), and train deep learning models to map one to the other. Although well intentioned, this approach often ignores a principled analysis of whether the input sensor data has enough information to predict the desired metric. We analyze the task of predicting blood pressure from PPG pulse wave analysis. Our review of the prior work reveals that many papers fall prey data leakage, and unrealistic constraints on the task and the preprocessing steps. We propose a set of tools to help determine if the input signal in question (e.g., PPG) is indeed a good predictor of the desired label (e.g., blood pressure). Using our proposed tools, we have found that blood pressure prediction using PPG has a high multi-valued mapping factor of 33.2% and low mutual information of 9.8%. In comparison, heart rate prediction using PPG, a well-established task, has a very low multi-valued mapping factor of 0.75% and high mutual information of 87.7%. We argue that these results provide a more realistic representation of the current progress towards to goal of wearable blood pressure measurement via PPG pulse wave analysis.

==> content/5_experiments.tex <==
\section{Experiments}

%For our analysis we use the dataset in majorly two ways, one is where we use an autoencoder on the raw waveform to reduce the dimensionality of the feature space and obtain meaningful bottleneck features and second is where we extract handcrafted features from prior literature like hr, hrv, systolic slope etc. 


    
% \end{enumerate}


==> content/8_conclusion.tex <==
\section{Conclusion}

Predicting blood pressure from PPG is attractive, as it would enable continuous, non-invasive and comfortable measurement. However, the relationship between the input (PPG) and output (BP) is not well understood. Data driven supervised learning approaches, often using highly parameterized neural networks, are popular. However, although well intentioned, they can fall prey to common pitfalls. We have shown that data leakage, aggressive constraints on the prediction task, calibration, and unrealistic preprocessing can lead to misleading claims and over-optimistic results. We propose two simple tools that help reveal how difficult the task of BP prediction is, showing how there are a large amount of multi-valued mapping and very low mutual information between the input signal and the output, whether using handcrafted or learned features. We encourage researchers using data-driven models to also apply these tools to their data to reduce the opportunity for bias and standard deviation results to mislead readers.
